SharpNet: Fast and Accurate Recovery of Occluding Contours in Monocular Depth Estimation

We introduce SharpNet, a method that predicts an accurate depth map for an input color image, with a particular attention to the reconstruction of occluding contours: Occluding contours are an important cue for object recognition, and for realistic integration of virtual objects in Augmented Reality, but they are also notoriously difficult to reconstruct accurately. For example, they are a challenge for stereo-based reconstruction methods, as points around an occluding contour are visible in only one image. Inspired by recent methods that introduce normal estimation to improve depth prediction, we introduce a novel term that constrains depth and occluding contours predictions. Since ground truth depth is difficult to obtain with pixel-perfect accuracy along occluding contours, we use synthetic images for training, followed by fine-tuning on real data. We demonstrate our approach on the challenging NYUv2-Depth dataset, and show that our method outperforms the state-of-the-art along occluding contours, while performing on par with the best recent methods for the rest of the images. Its accuracy along the occluding contours is actually better than the `ground truth' acquired by a depth camera based on structured light. We show this by introducing a new benchmark based on NYUv2-Depth for evaluating occluding contours in monocular reconstruction, which is our second contribution.

==> supplementary_materials.tex <==
%%% To put in supplementary materials

\begin{table*}
	\begin{center}
		\begin{tabular}{|l||ll|ll|lll|}
			\hline
			Method & $\epsilon_{PE}^{plan} (cm) \downarrow$    & 
			$\epsilon_{PE}^{orie} (\deg) \downarrow$ & 
			$\epsilon_{DBE}^{acc} 
			(px) \downarrow$    & $\epsilon_{DBE}^{comp} (px) 
			\downarrow $ & 
			$\epsilon_{DDE}^{0} \uparrow$ & $\epsilon_{DDE}^{-} 
			\downarrow $ & 
			$\epsilon_{DDE}^{+} \downarrow $\\ \hline\hline
			Eigen \cite{Eigen14} & 6.65 & 25.62 & 5.48 & 70.31 & 72.06 
			& 25.71 
			& 2.23 \\
			Eigen \cite{Eigen2015PredictingDS} (AlexNet) & 6.34 & 21.74 
			& 4.57 
			& 46.52 & 78.24 & 17.86 & 3.90 \\
			Eigen \cite{Eigen2015PredictingDS} (VGG) & 4.93 & 17.18 & 
			4.51 & 
			43.64 & 80.73 & 17.47 & 1.80 \\
			Laina \cite{Laina2016DeeperDP} & 5.71 & 18.49 & 6.89 & 
			40.48 & 
			81.65 & 15.91 & 2.43 \\
			Liu \cite{LiuPAMI15} & 6.82 & 29.22 & 3.57 & 31.75 & 80.46 
			& 13.26 
			& 6.28 \\
			Li \cite{LiICCV17} & 6.22 & 20.17 & 3.68 & 36.27 & 84.13 & 
			12.49 & 
			3.38 \\
			Ours & 8.21 & 21.00 & \textbf{2.31} & 58.26 & 
			\textbf{85.95} & 
			\textbf{6.49}  & 7.56 \\ \hline
		\end{tabular}
	\end{center}
	\caption{Evaluation on metrics proposed by 
	\cite{Koch2018EvaluationOC} on 
	their dataset iBims-v1}
\end{table*}

\paragraph{Comparison with the iBims-v1 benchmark.}

\begin{table}[t]
	\begin{center}
		\resizebox{\linewidth}{!}{
			\begin{tabular}{|l|lll|lll|}
				\hline
				Method          & rel  & log  & rmse  & $\delta_1$ & $\delta_2$ 
& $\delta_3$ \\ \hline\hline
				Eigen           & 0.32 & 0.17 & 1.55  & 0.36   & 0.65   & 
0.84   \\ 
				Eigen (AlexNet) & 0.30 & 0.15 & 1.38  & 0.40   & 0.73   & 
0.88   \\ 
				Eigen (VGG)     & 0.25 & 0.13 & 1.26  & 0.47   & 0.78   & 
0.93   \\ 
				Laina           & 0.25 & 0.13 & 1.20  & 0.50   & 0.78   & 
0.91   \\ 
				Liu             & 0.30 & 0.13 & 1.26  & 0.48   & 0.78   & 
0.91   \\ 
				Li              & \textbf{0.22} & 0.11 & 1.07  & 0.59   & 
0.85   & 0.95   \\ 
				Ours            & 0.26 & \textbf{0.10} & \textbf{0.952} & 
\textbf{0.63} &  \textbf{0.87}   & 0.94   \\ \hline
		\end{tabular}}
	\end{center}
	\caption{Evaluation on depth estimation on the iBims-v1 dataset (our method 
was trained on \cite{Zhang2016pbrs} dataset then finetuned on NYUv2, while 
others were trained on NYUv2 only}
\end{table}


\paragraph{Comparison for scene reconstruction}

\begin{figure*}[t]
	\begin{center}
		\includegraphics[width=\linewidth]{augmentation_new2.pdf}
	\end{center}
	\caption{We present some augmentation on images and display the ability of 
	our method to retrieve sharp and accurate occlusion boundaries on depth 
	maps, making it suitable for augmented reality}
	\label{fig:augmentation}
\end{figure*}
